A spin-optomechanical quantum interface enabled by an ultrasmall mechanical and optical mode volume cavity

We propose a coherent mechanical interface between defect centers in diamond and telecom optical modes. Combining recent developments in spin-mechanical devices and optomechanical crystals, we introduce a 1D diamond nanobeam with embedded mechanical and electric field concentrator with mechanical and optical mode volumes $V_\mathrm{mech}/\Lambda_\mathrm{p}^3\sim 10^{-5}$ and $V_\mathrm{opt}/\lambda^3\sim 10^{-3} $, respectively. By placing a Group IV vacancy in the concentrator we demonstrate exquisitely high spin-mechanical coupling rates approaching 40 MHz, while retaining high acousto-optical couplings. We theoretically show that such a device, used in an entanglement heralding scheme, can provide high-fidelity Bell pairs between quantum repeaters. Using the mechanical interface as an intermediary between the optical and spin subsystems, we are able to directly use telecom optics, bypassing the native wavelength requirements of the spin. As the spin is never optically excited or addressed, we do not suffer from spectral diffusion and can operate at higher temperatures (up to 40 K), limited only by thermal losses. We estimate that based on these metrics, optomechanical devices with high spin-mechanical coupling will be a useful architecture for near-term quantum repeaters.

==> scratch.tex <==


\clearpage
\onecolumngrid 
\appendix
\section{Scratch Notes}
\begin{align}
  \dot{\hat{a}} & = i \left[g \hat{a} \hat{b} + \mathrm{H.c.}, \hat{a}\right] = -ig^*\hat{b}^\dagger \\
  \dot{\hat{b}} & = i \left[g \hat{a} \hat{b} + \mathrm{H.c.}, \hat{b}\right] = -ig^*\hat{a}^\dagger
\end{align}
therefore
\begin{align}
  \hat{a}(t) & = \cosh(|g|t) \hat{a}(0) - i \frac{g^*}{|g|} \sinh(|g|t) \hat{b}^\dagger(0) \\
  \hat{b}(t) & = \cosh(|g|t) \hat{b}(0) - i \frac{g^*}{|g|} \sinh(|g|t) \hat{a}^\dagger(0)
\end{align}

With loss:

\begin{align}
  \hat{H} & = \hbar g \hat{a} \hat{b} + \mathrm{H.c.} - \frac{i \hbar}{2}\gamma_\mathrm{e} \hat{a}^\dagger \hat{a}
\end{align}
therefore
\begin{align}
  \dot{\hat{a}} & = i \left[g \hat{a} \hat{b} + \mathrm{H.c.} - \frac{i}{2}\gamma_\mathrm{e} \hat{a}^\dagger \hat{a}, \hat{a}\right] = -ig^*\hat{b}^\dagger - \frac{\hbar\gamma_\mathrm{e}}{2}\hat{a} \\
  \dot{\hat{b}} & = i \left[g \hat{a} \hat{b} + \mathrm{H.c.} - \frac{i}{2}\gamma_\mathrm{e} \hat{a}^\dagger \hat{a}, \hat{b}\right] = -ig^*\hat{a}^\dagger
\end{align}
therefore
\begin{align}
  \ddot{\hat{a}} & =  |g|^2\hat{a} - \frac{\gamma_\mathrm{e}}{2}\dot{\hat{a}} \\
\end{align}
therefore
\begin{align}
  \hat{a}(t) & = e^\frac{-\gamma_\mathrm{e} t}{4} \left( \hat{a}(0) \cosh(g't) + \hat{B} \sinh(g't)\right) \\
  g' & = \sqrt{|g|^2 + \frac{\gamma_\mathrm{e}^2}{16}} \\
  \hat{B} & = \frac{-ig^*\hat{b}^\dagger(0) - \frac{\gamma_\mathrm{e}}{4} \hat{a}(0)}{g'}
\end{align}
therefore
\begin{equation}
\begin{split}
  \hat{a}(t) & = e^\frac{-\gamma_\mathrm{e} t}{4} \hat{a}(0) \left(\cosh(g't) -\frac{\gamma_\mathrm{e}}{4g'}\sinh(g't)\right) \\
             & + e^\frac{-\gamma_\mathrm{e} t}{4} \hat{b}^\dagger(0) \frac{-ig^*}{g'} \sinh(g't) \\
  \hat{b}(t) & = e^\frac{-\gamma_\mathrm{e} t}{4} \hat{a}^\dagger(0) \frac{-ig^*}{g'} \sinh(g't) \\
             & + e^\frac{-\gamma_\mathrm{e} t}{4} \hat{b}(0) \left(\cosh(g't) +\frac{\gamma_\mathrm{e}}{4g'}\sinh(g't) \right)
\end{split}
\end{equation}
therefore
\begin{align}
  \langle\gamma_\mathrm{e}\hat{a}^\dagger\hat{a}\rangle_{(t)} & = \gamma_\mathrm{e} e^\frac{-\gamma_\mathrm{e} t}{2}\frac{|g|^2}{{g'}^2}\sinh(g't)^2
\end{align}
which was verified numerically with Lindblad's equation

Also we get (if we assume $g$ is imaginary, in order to simplify the expression so that we do not have to deal with the momentum operator)
\begin{equation}
\begin{split}
  \hat{X}^2_a(t) + \hat{X}^2_b(t) & =
    \frac{1}{2}\left(\hat{a}(t)+\hat{a}^\dagger(t)\right)^2 + \frac{1}{2}\left(\hat{b}(t)+\hat{b}^\dagger(t)\right)^2 \\ 
  = & \text{ math stuff...} \\
  = & e^{-\frac{\gamma_\mathrm{e} t}{2}}\left[\left(C_a\hat{X}_a(0) + D_b \hat{X}_b(0)\right)^2 + \left(C_b\hat{X}_b(0) + D_a \hat{X}_a(0)\right)^2\right]
\end{split}
\end{equation}
where
\begin{align}
  C_a &= \frac{\gamma_\mathrm{e}}{4g'} \sinh{\left({g}' t \right)} - \cosh{\left({g}' t \right)} \\ 
  C_b &= \frac{\gamma_\mathrm{e}}{4g'} \sinh{\left({g}' t \right)} + \cosh{\left({g}' t \right)} \\ 
  D_a &= \frac{ig}{g'}\sinh{\left({g}' t \right)} \\ 
  D_b &= -\frac{ig}{g'}\sinh{\left({g}' t \right)}
\end{align}

https://arxiv.org/abs/1401.4118

Writing amplitudes in the Fock basis:
%Time evolution of our system is given by
%\begin{align}
%    S &= e^{-ig\hat{a}\hat{b} - ig^*\hat{a}^\dagger\hat{b}^\dagger - \frac{\gamma}{2}\hat{a}^\dagger\hat{a}}\\
%    &= \sum_n\frac{1}{n!}(-ig\hat{a}\hat{b}-ig\hat{a}^\dagger\hat{b}^\dagger - \frac{\gamma}{2}\hat{a}^\dagger\hat{a})^n
%\end{align}

Tensor product of vacuum states with squeezing:
\begin{align}
    \psi_{00}(\hat{X}_a(t),\hat{X}_b(t)) &=\frac{1}{\sqrt{\pi}}e^{-(\hat{X}_a(t)^2+\hat{X}_b(t)^2)/2}\\
    &=\frac{1}{\sqrt{\pi}}e^{-\left[(C_a\hat{X}_a(0)+D_b\hat{X}_b(0))^2 + (C_b\hat{X}_b(0) + D_a\hat{X}_a(0))^2\right]\exp(-\gamma t/2)}
\end{align}

Inner product with squeezed states $\psi_{a(b)}(X_{a(b)}) = \frac{1}{\pi^{1/4}}e^{-(X_{a(b)}-\alpha_{a(b)}\sqrt{2})^2/2}$:
\begin{align}
    \bra{\alpha_a\alpha_b}\ket{sq} &= \iint dX_a dX_b \psi_{00}(X_a,X_b)\psi_a^*\psi_b^*\\
    &=\frac{1}{\pi}\iint dX_a dX_b e^{-((C_a^2 + D_a^2)\hat{X}_a^2 + 2(C_a D_b + D_a C_b) \hat{X}_a \hat{X}_b + (C_b^2 + D_b^2)\hat{X}_b^2)/2} \\
    &\;\;\;\times e^{-\frac{1}{2}(X_a^2 - 2\alpha_a\sqrt{2}X_a + 2\alpha_a^2) - \frac{1}{2}(X_b^2 - 2\alpha_b\sqrt{2}X_b + 2\alpha_b^2)}\\
    &=\frac{1}{\pi}\iint dX_a dX_b e^{-\frac{1}{2}(C_a^2 + D_a^2 + 1)X_a^2 - ((C_a D_b + D_a C_b) X_b - \alpha_a \sqrt{2})X_a}\\
    &\;\;\; \times e^{-\frac{1}{2}(C_b^2 +D_b^2 + 1)X_b^2 + \alpha_b\sqrt{2}X_b - \alpha_a^2 - \alpha_b^2}
\end{align}
Using $\int e^{-ax^2 + bx + c}dx = \sqrt{\frac{\pi}{a}}e^{-\frac{b^2}{4a} + c}$,  integrate over $X_a$ and $X_b$:
 
\begin{align}
    \bra{\alpha_a \alpha_b}\ket{sq} &= 2\sqrt{\frac{1}{((1 + A) (1 + B) - C^2)}}e^{\left[-\alpha_a^2 - \alpha_b^2 + \frac{\alpha_a^2 (1 + B) + \alpha_b^2 (1 + A) - 2 \alpha_a \alpha_b C}{1 + A + B + A B - C^2}\right]\exp(-\gamma t/2)}.
\end{align} 
Here, $A = C_a^2 + D_a^2$, $B = C_b^2 + D_b^2$, and $C = C_a D_b + D_a C_b$.

Simplify by substituting definitions for $C_i$ and $D_i$:


%Is there something wrong with this math? I can't get the expression to a form where the a and b subscripts are interchangeable like I think they should be, since the initial integral is symmetric
%Note to self: rely on Mathematica more but just use it smartly

Decompose in the Fock basis and solve for $\alpha_a$ and $\alpha_b$:
\begin{align}
    \ket{\alpha} = \sum_ne^\frac{-\alpha^2}{2}\frac{\alpha^n}{\sqrt{n!}}\ket{n}
\end{align}

Tensor product of coherent states in the Fock basis:

\begin{align}
    \ket{\alpha_a, \alpha_b } = \sum_{m,n}e^{-\frac{\alpha_a^2}{2} - \frac{\alpha_b^2}{2}}\frac{\alpha_a^n\alpha_b^m}{\sqrt{n!m!}}\ket{n, m}
\end{align}

Inner product using Fock states:
\begin{align}
    \sum_{m,n} \bra{n,m} \frac{\alpha_a^n\alpha_b^m}{\sqrt{n!m!}}e^{-\frac{\alpha_a^2}{2} - \frac{\alpha_b^2}{2}}\ket{sq} = 2\sqrt{\frac{1}{((1 + A) (1 + B) - C^2)}}e^{\left[-\alpha_a^2 - \alpha_b^2 + \frac{\alpha_a^2 (1 + B) + \alpha_b^2 (1 + A) - 2 \alpha_a \alpha_b C}{1 + A + B + A B - C^2}\right]\exp(-\gamma t/2)}
\end{align}

Given the form of our Hamiltonian, assume $n = m$ and identical coherent states. (Justified because the $\hat{a}\hat{b}$ and $\hat{a}^\dagger\hat{b}^\dagger$ operators do not change $n$ and $m$ relative to each other, and the $\hat{a}^\dagger\hat{a}$ operator does not change the optical photon number $n$, only reads it out) Then

\begin{align}
    \sum_{n} \bra{n n}\frac{\alpha^{2n}}{n!}\ket{sq} &= 2\sqrt{\frac{1}{((1 + A) (1 + B) - C^2)}}e^{\left[-2\alpha^2 + \alpha^2\left(\frac{2 + A + B - C}{1 + A + B + AB - C^2}\right)\right]\exp(-\gamma t)}e^{\alpha^2}\\
    &= 2\sqrt{\frac{1}{((1 + A) (1 + B) - C^2)}}\sum_n \frac{1}{n!}\left[ \left(-2 + \frac{2 + A + B - C}{1 +A + B + AB - C^2}\right)e^{-\gamma t/2} + 1\right]^n\alpha^{2n}.
\end{align}

Therefore, we find our number state coefficients as a function of time are
\begin{align}
    \bra{nn}\ket{sq} = 2 \sqrt{\frac{1}{(1 + A)(1 + B) - C^2}}\left[ \left(-2 + \frac{2 + A + B - C}{1 +A + B + AB - C^2}\right)e^{-\gamma t/2} + 1\right]^n
\end{align}

%Check against numerical simulations I guess?

\section{Radiative Coupling to a Cold Bath}
\citep{Jiang proposal for heralded MW-OPT generation}
\citep{Triply resonant cavity electro-optomechanics}
Because we are operating our input pump laser in the non-classical regime, we expect thermal heating in the microwave mode of our transducer. Previous studies (\citep{people above}) have proposed operating the device at a higher temperature stage stage (i.e. 1 K) while strongly coupling to a cold temperature "bath" (i.e. 10 mK) to increase the device's power handling capacity.
To incorporate this radiative cooling proposal in our entanglement scheme, we can operate our electro-optic transducer at a 1 K stage while coupling to a 10 mK dilution refrigerator stage. Suppose that our transducer operates at a microwave mode on the order of $\omega_m \sim 1$ GHz. At 1 K, the thermal mode occupancy will be $n_{1K} = \frac{1}{e^{\hbar \omega_m/ k_b T} + 1} \approx 0.488$. In contrast, the thermal mode occupancy at 10 mK will be $n_{10mK} \approx 0.008$. Suppose that our microwave mode couples to its 1 K environmental bath with intrinsic coupling rate $\kappa_i$ and couples to the 10 mK bath with extrinsic coupling rate $\kappa_e$. Then the microwave cavity mode occupancy will be given by \citep{Hong Tang radiative coolign paper}
\begin{align}
    n_{mode} = \frac{\kappa_i n_{1K} + \kappa_{e}n_{10mK}}{\kappa_i + \kappa_e} = n_{1K} - \frac{\kappa_e}{\kappa_i + \kappa_e}(n_{1K} - n_{10mK}).
\end{align}
 In the regime where $\kappa_e >> \kappa_i$, this effectively reduces the microwave mode occupancy of our cavity by $\sim 0.48$ noise photons. Coupling rate ratios of $\kappa_e/\kappa_i = 4.4$ have been achieved. Using this ratio, for operation between 1 and 10 GHz, we can expect a noise photon suppression of around 0.3-0.4 by implementing radiative coupling.
 

\section{Notes for discussion}

By current estimates, fault-tolerant quantum computing with known useful applications will require large numbers (100s to 1000s) of logical qubits encoded in perhaps millions of physical qubits. It is presently unclear how any given physical system can supply these resources. One appealing approach, however, is in hybrid quantum systems, which have the potential to optimally combine the unique advantages of disparate physical qubits. However, standing in the way of building scalable hybrid quantum quantum information processors is the need for efficient, fast, and high-fidelity quantum interfaces. This need is perhaps most pressing in superconducting circuit-based quantum information processos, which have high-fidelity and high-speed  initialization and logic gates, but face critical scaling challenges in improving qubit (i) coherence times, (ii) long-range connectivity, (iii) qubit number, and (iv) readout fidelity.
Here we introduce a solution to these bottlenecks in the form of a high-speed, high-fidelity quantum state transducer between superconducting qubits and artificial atom (AA) spins, mediated via an acoustic bus connected by piezoelectric transducers. Applied to present-day experimental parameters for superconducting circuit qubits and diamond silicon vacancy centers in an optimized phononic cavity, we estimate quantum state transduction with fidelity exceeding 99\% at a MHz-scale bandwidth. By combining the complementary strengths of superconducting circuit quantum computing and artificial atoms, we estimate that the superconducting-AA architecture will combine high-speed, high-fidelity qubit gates with long-lived quantum memory, high-fidelity measurement, large qubit number, reconfigurable qubit connectivity, and high-fidelity state and gate teleportation across optical quantum networks. 
To summarize our results, our proposed hybrid architecture combines the favorable attributes of AA quantum memories with SC quantum information processors, including:
QPU with high-speed, high-fidelity quantum gates already demonstrated in SC machines
Phononic bus connecting with high coherence, reconfigurable through random-access switch links in acoustic or superconducting bus 
High-capacity QM in AA electron/nuclear spins with long coherence times (>  minutes) and perhaps hours
High-fidelity quantum state readout, 
High-fidelity long-range state and gate teleportation by heralded entanglement in quantum networks

\section{Dark Counts}

Let us denote the state of the system at time $t$ prior to a detection by $|\psi\rangle$. The rate of true detections at time $t$ is $r_{t} = \langle \psi|a^\dagger a|\psi\rangle$. When a true detection occurs at time $t$ the state of the system becomes 
\begin{align}
    |\tilde{\psi}\rangle = \frac{a |\psi\rangle}{\sqrt{r_t}} . 
\end{align}
The dark count rate is $d$. When a photo-count occurs, the posterior probability that it is a true detection is 
\begin{align}
   p_t = r_t/(r_t + d) .  
\end{align}
and that it is a dark count is 
\begin{align}
   q_t = d/(r_t + d) .  
\end{align}
So the post-detection state is 
\begin{align}
    \rho = p_t |\psi\rangle \langle \psi | + q_t |\tilde{\psi}\rangle \langle \tilde{\psi} |  
\end{align} 

